On approximate pure Nash equilibria in weighted congestion games with polynomial latencies

We study natural improvement dynamics in weighted congestion games with polynomial latencies of maximum degree $d\geq 1$. We focus on two problems regarding the existence and efficiency of approximate pure Nash equilibria, with a reasonable small approximation factor, in these games. By exploiting a simple technique, we firstly show that such a game always admits a $d$-approximate potential function. This implies that every sequence of $d$-approximate improvement moves by the players leads to a $d$-approximate pure Nash equilibrium. As a corollary, we also obtain that, under mild assumptions on the structure of the players' strategies, the game always admits a constant approximate potential function. Secondly, using a simple potential function argument, we are able to show that a $(d+\delta)$-approximate pure Nash equilibrium of cost at most $(d+1)/(d+\delta)$ times the cost of an optimal state always exists, for $\delta\in [0,1]$.

==> tree.tex <==
\psset{radius=3pt,levelsep=1cm, tnpos=r}

\begin{figure*}[h]
\centering

%\pstree[thislevelsep=0,edge=none,levelsep=2.5cm]{\Tn}{%
%\pstree{\TR{Player 1}}{\pstree{\TR{Player 2}}{\TR{Player 3}}}

\pstree{\Tn}
{


\psset{linestyle=dashed, nodesep=3pt, labelsep=25pt}
\pstree[edge=none]{\TR{\textrm{Resource}}\tlput{(\texttt{Level $0$})}}
{
	\pstree[edge=\ncline]{\TR{\textrm{Players}}}
	{
			\pstree[edge=none]{\TR{\textrm{Resources}}\tlput{(\texttt{Level $1$})}}
			{
					\pstree[edge=\ncline]{\TR{\textrm{Players}}}
					{
							\pstree[edge=none]{\TR{\textrm{Resources}}\tlput{(\texttt{Level $2$})}}
							{
									\pstree[edge=\ncline]{\TR{\textrm{Players}}}
									{
											\pstree[edge=none,levelsep=2cm]{\TR{\textrm{Resources}}\tlput{(\texttt{Level $3$})}}
											{
												\pstree[edge=\ncline,levelsep=1cm]{\TR{\textrm{Players}}}
												{
													\TR{\textrm{Resources}}\tlput{(\texttt{Level $q$})}
												}
											}
									}
							}
					}
			}
	}
}



\psset{linestyle=solid,nodesep=1pt, labelsep=7pt}
\pstree{\Tf~{$(1,\d)$}}
{ 
	
	\pstree{\TC*}{ % left sub-tree
		\pstree{\Tf}{
			\pstree{\TC*}
			{ 
				\pstree{\Tf}
				{
					\pstree{\TC*}
					{
						\pstree[edge=none, levelsep=2cm]{\Tf[name=LU]}
						{
							\pstree[edge=\ncline, levelsep=1cm]{\TC*[name=LL]}
							{
								\Tf
							}
							\pstree[edge=\ncline, levelsep=1cm]{\TC*[name=AA]}
							{
								\Tf
							}
						}
					}
					\pstree{\TC*}
					{
						\Tf
					}
				}
			}
			\pstree{\TC*}
			{ 
				\pstree{\Tf}
				{
					\pstree{\TC*}
					{
						\Tf
					}
					\pstree{\TC*}
					{
						\Tf
					}
				}
			}
		}
	} % end left


	\pstree{\TC*~{$\w$}}{ % right sub-tree
		\pstree{\Tf~{$(1,\d)$}}{
			\pstree{\TC*}
			{ 
				\pstree{\Tf}
				{
					\pstree{\TC*}
					{
						\Tf
					}
					\pstree{\TC*}
					{
						\Tf
					}
				}
			}
			\pstree{\TC*~{$\frac{\w}{2} + \epsilon$}}
			{ 
				\pstree{\Tf~{$(1,\d)$}}
				{
					\pstree{\TC*}
					{
						\Tf
					}
					\pstree{\TC*~{$\frac{\w}{4} + 2\epsilon$}}
					{
						\pstree[edge=none, levelsep=2cm]{\Tf[name=RU]~{$(1,\d)$}}
						{
							\pstree[edge=\ncline, levelsep=1cm]{\TC*[name=BB]}
							{
								\Tf
							}
							\pstree[edge=\ncline, levelsep=1cm]{\TC*[name=RR]~{$\frac{\w}{2^{q-1}} + (q-1)\epsilon$}}
							{
								\Tf~{$(4,\d)$}
							}
						}
					}
				}
			}
		}
	} % end right
	
}

}

\ncline[linestyle=dotted, nodesep=2cm]{AA}{BB}
\ncline[linestyle=dotted, nodesep=10pt]{LL}{LU}
\ncline[linestyle=dotted, nodesep=10pt]{RR}{RU}

 \caption{Lower bound instance $\G_q$.}\label{fig:LB}
\end{figure*}
